Multi-Time Attention Networks for Irregularly Sampled Time Series

Irregular sampling occurs in many time series modeling applications where it presents a significant challenge to standard deep learning models. This work is motivated by the analysis of physiological time series data in electronic health records, which are sparse, irregularly sampled, and multivariate. In this paper, we propose a new deep learning framework for this setting that we call Multi-Time Attention Networks. Multi-Time Attention Networks learn an embedding of continuous-time values and use an attention mechanism to produce a fixed-length representation of a time series containing a variable number of observations. We investigate the performance of this framework on interpolation and classification tasks using multiple datasets. Our results show that the proposed approach performs as well or better than a range of baseline and recently proposed models while offering significantly faster training times than current state-of-the-art methods.

==> applications.tex <==
\section{Applications}
In this section, we present two applications of our Time Attention based encoder-decoder framework - \emph{Interpolation} and \emph{Supervised Learning}. Given an sparse and irregularly sampled time series $(\mbf{x}, \mbf{t})$, the goal of the interpolation is to infer the values at unobserved time points $\mbf{t}'$. The interpolations can be computed using equations shown in section \ref{sec:enc-dec}.

Our encoder-decoder framework can also be used to perform supervised learning from multivariate, sparse and irregularly sampled time series. In order to achieve this, we augment the learning objective to include the supervised learning term. For classification case with target label $y_n$ for data case $n$, the supervised learning loss is defined as below:
%
\begin{align}
\label{eq:classif}
\nonumber
& \mathcal{L}_{\text{supervised}} (\theta, \gamma, \phi) = \sum_{n=1}^N \;\frac{1}{ \sum_d L_{dn}}\Big(\mathbb{E}_{q_{\gamma}(\mbf{z}_1, \cdots, \mbf{z}_T|\mbf{x}_n, \mbf{t}_n)} [\log p_{\theta}(\mbf{x}_n| \mbf{z}_1, \cdots, \mbf{z}_T, \mbf{t}_n) ] \\
&\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;-  \KL(q_{\gamma}(\mbf{z}_1, \cdots, \mbf{z}_T | \mbf{x}_n, \mbf{t}_n) || p(\mbf{z}_1, \cdots, \mbf{z}_T))\Big) \nonumber\\
&\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;+ \mathbb{E}_{q_{\gamma}(\mbf{z}_1, \cdots, \mbf{z}_T|\mbf{x}_n, \mbf{t}_n)} \log p_\phi(y_n|\mbf{z}_1, \cdots, \mbf{z}_T) 
\end{align}
%
where $\phi$ parameterizes the classifier. We use a GRU followed by 2-layer fully connected network as the classifier. 
 Note that the encoder does not depend on the target label $y_n$. This provides the flexibility of using a pre-trained encoder or learn everything jointly or perform semi-supervised learning with only available labels. 

The ELBO component in the learning objective described in Equation \ref{eq:classif} acts as a regularization term and avoids overfitting. In practice, we use a constant factor in front of the supervised loss component to control the trade-off between the supervised loss component and the regularization term. At test time, predictions are made using latent vectors as:
%
\begin{align}
    y^* = \argmax_y \; \mathbb{E}_{q_{\gamma}(\mbf{z}_1, \cdots, \mbf{z}_T|\mbf{x}, \mbf{t})} \log p_\phi(y|\mbf{z}_1, \cdots, \mbf{z}_T) 
\end{align}



==> broader_impacts.tex <==
\section{Broader Impact}

This work is motivated by data analytic challenges that arise when modeling and learning from missing and irregularly sampled data. Sparse and irregular sampling is one of the major challenges when working with time series collected in the healthcare setting as part of  routine care. Both the in-patient and out-patient settings result in similarly structured data. In this work, our  evaluation uses the MIMIC-III and PhysioNet data sets, which consist of intensive care unit records that exhibit significant incompleteness and irregular sampling.  The ability to leverage such data via machine learning models that can efficiently and appropriately represent uncertainty due to incompleteness has the potential to lead to more accurate and scalable clinical decision support tools, which can in turn directly impact quality of care and health outcomes for the population at large. 

==> model.tex <==
\section{Multi-Time Attention Networks}

In this section, we present the proposed Multi-Time Attention Network (\acro) model. We begin by presenting notation followed by the model architecture and learning criteria. 

\paragraph{Notation:}
In the case of a supervised learning task, we let $\mathcal{D}=\{(\mbf{s}_n,y_n) | n=1,...,N\}$ represent a data set containing
$N$ data cases. An individual data case consists of
a single target value $y_n$ (discrete for classification), as well as a $D$-dimensional, sparse and irregularly
sampled multivariate time series $\mbf{s}_n$. Different dimensions $d$ of the multivariate
time series can have observations at different times, as well as different total
numbers of observations $L_{dn}$. Thus, we represent time series $d$ for data case $n$ as a tuple
$\mbf{s}_{dn}=(\mbf{t}_{dn}, \mbf{x}_{dn})$  where $\mbf{t}_{dn}=[t_{1dn},...,t_{L_{dn}dn}]$
is the list of time points at which observations are defined and 
$\mbf{x}_{dn}=[x_{1dn},...,x_{L_{dn}dn}]$ is the corresponding list of observed values. In the case of an unsupervised task such as interpolation, each data case will consist of a multivariate time series $\mbf{s}_n$ only. We drop the data case index $n$ for brevity when the context is clear.

%\paragraph{Model Architecture:}
%We introduce time attention network for modeling the irregularly sampled time series data.  It requires learning a vector representation of time. Time attention network 
%interpolates the multivariate, sparse, and irregularly
%sampled input time series against a set of evenly spaced %reference time points.  
%Our overall model architecture consists of a encoder and %decoder model. 
%Both the encoder and decoder consist of time attention %network for handling the 
%%sparse and irregularly sampled data. The parameters of our %model are learned by maximizing the 
%variational lower bound on the log marginal likelihood (the evidence lower bound or ELBO).
% We describe the components of the model in detail below.
%Figure 1 shows the architecture of the proposed model.

\paragraph{Time Embeddings}
Time Attention Networks are based on embedding continuous time points into a vector space. We generalize the notion of a positional encoding used in transformer-based models to continuous time. Specifically, we define a $d_k$-dimensional embedding of continuous time as: 

\begin{equation}
    \phi(t)[i] = \begin{cases}
               \omega_0 t + \alpha_0, \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \text{if} \;\;\;\; i = 0\\
               \sin(\omega_i t + \alpha_i), \;\;\;\;\;\;\;\;\;\;\;  \text{if} \;\;\;\; 0 < i < d_k         
           \end{cases}
\end{equation}
where $\omega_i$'s and $\alpha_i$'s and are learnable parameters. The periodic terms capture the periodicity in the time series. In this case, $\omega_i$ and $\alpha_i$ represent the frquency and phase of the sine function. The linear term, on the other hand, can capture non-periodic patterns dependent on the progression of time. For a given difference $\delta$, $\phi(t + \delta)$ can be represented as a linear function of $\phi(t)$. Learning this time embedding function is equivalent to using a one-layer fully connected network with a sine function non-linearity to map the time values into a higher dimensional space. 

By contrast, the positional encoding used in transformer models is defined only for discrete positions.  We note that our time embedding actually subsumes positional encodings through the mapping: 
\begin{equation*}
    \omega_i, \alpha_i = \begin{cases}
            \frac{1}{10000^{2i/d_k}}, 0\;, \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \text{if $i$ is even} \\
            \omega_{i-1}, \frac{\pi}{2} \;, \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \text{if $i$ is odd}        
           \end{cases}
\end{equation*}
Since, positional encodings do not contain any linear term, $\omega_0 = 0$ and $\phi_0 = 0$. Finally we note that we do not concatenate the time embedding with other embeddings or representations as in transformers. Instead, we use the learned time embeddings as key and query points in an attention mechanism, which we describe next. 

\paragraph{Time Attention:}
\label{sec:tan}
%cite{Attention paper}\\
We next define a time attention mechanism that uses time embeddings as queries and keys. When given a query as input, the mechanism matches the query to the keys and returns a similarity weighted average of the values associated with the keys. The weight is given by a scaled dot product of the query with each key. The time attention function for an irregularly sampled univariate time series $\mbf{s}=\{(t_i, x(t_i))_{i=1}^L\}$ at time $t$ is defined as: 
%
\begin{align}
\label{eq:interp}
    \hat{x}(t,\mbf{s}) = \sum_{i = 1}^L \kappa(t, t_i)\, x(t_i),\;\;\;\;  
      \kappa(t, t_i) = \softmax \bigg(\frac{q_t\,k_{t_i}^T}{\sqrt{d_k}}\bigg) 
\end{align}
%
%In this work, we introduce Time Attention function, which interpolate the irregularly sampled time series on a set of fixed reference points. We define keys and queries to be learnable embeddings of time.
%
where $\hat{x}(t)$ is the interpolated output at time $t$;  $q_t = \phi(t)W^Q \text{ and } k_{t} = \phi(t)W^K$ are linear projections of the learnable embedding function $\phi(\cdot ) \in \mathbb{R}^{d_k}$ for query point $t$ and key point $t_i$; $d_k$ is the dimension of the embedding; and $W^Q \in \mathbb{R}^{d_k\times d_k}$ and $W^K \in \mathbb{R}^{d_k\times d_k}$ are the learnable weight parameter matrices defining the linear projections. We use a scaling factor $\frac{1}{\sqrt{d_k}}$ to normalize the dot product to counteract the growth in the dot product magnitude with increase in the dimension $d_k$.
$t$ is referred to as the query point, the $t_i$'s are the keys and the $x(t_i)$'s are the values.

Equation \ref{eq:interp} is similar to learning an interpolation using a pre-specified kernel function $\kappa (\cdot, \cdot)$. In this work, we define a linear kernel using scaled dot product of time embeddings. Learning the time embeddings provides our model with flexibility to learn the kernel function. In fact, given large enough $d_k$, the dot product of time embeddings can approximate the RBF kernel. 

In the multivariate case, we compute the interpolant $\hat{x}_d(t)$ for each dimension $d$ independently according to Equation \ref{eq:interp}. The required computations can be parallelized using masking variables to deal with unobserved dimensions. Finally, we note that the time attention network does not depend on the order of $(t_i, x_i)$ tuples and hence it is permutation invariant as required.

%In practice, we parallelize the process of computing the time attention function for a multivariate, sparse and irregularly sampled time series on a set of query points. In order to do this efficiently, we introduce mask variables to indicate whether variables are missing or observed.
%i.e. $m_{td} = 1 \text{ if } x_{td} \text{ is observed, else } 0$. 

%Note that the multivariate irregularly sampled time series can be transformed into a fixed length sequence using the mask variables. For a $D$-dimensional time series, we can pack together all the observations, time points and mask indicators in $V \in \mathbb{R}^{D\times L}$, $k \in \mathbb{R}^{D \times L}$  and $M \in \mathbb{R}^{D \times L}$ respectively where $L = \max_d L_d$. Time Attention function for a set of $T$ reference points packed into $q \in  \mathbb{R}^{T}$ can be computed simultaneously as:
%
%\begin{align}
%    \text{TAF}_W(q, k, V) =  \softmax\bigg(\frac{(QW^Q) (KW^K)^T \odot M}{\sqrt{d_k}}\bigg)\,V
%\end{align}
%
%where $Q \in  \mathbb{R}^{T \times d_k}$ is the packed embedding of the query time points, $K \in \mathbb{R}^{D \times L \times d_k}$ is the packed embedding of observed time points, $W = \{W^Q, W^K\}$ denote the parameters of the Time Attention network and $\odot$ represent the element wise multiplication. We mask the scaled dot product values corresponding to the missing/unobserved values and remove them from the computation of softmax scores. We achieve this by replacing the dot product values with a very large negative number at locations corresponding to missing values. The interpolations produced by time attention function only uses the observed time points and corresponding values for each dimension of the multivariate time series. Finally, we note that Time Attention network does not depend on the order of $(t, x)$ tuples and hence it is permutation invariant.

%\begin{property}
%Time Attention Network is permutation invariant. 
%\end{property}
 

% Scaled-dot product of two time embeddings quantify the similarity or distance between those time points similar to a kernel function. It can be interpreted as learning the kernel function defined by the time embedding without actually specifying the kernel. 
% This can also be interpreted as learning the infinite dimensional basis function?
% Equivalence to a kernel interpolation except that there is no need to define the kernel function. 


% Let $K \in \mathbb{R}^{D \times L \times d_k}$ be the packed embedding of key, then Time Attention function on a set of queries $Q \in  \mathbb{R}^{T \times d_k}$ (T reference points) can be computed simultaneously:
% \begin{align}
%     \text{TAF}(Q, K, V) =  \softmax\bigg(\frac{(QK^T) \odot M}{\sqrt{d_k}}\bigg)\,V
% \end{align}


\paragraph{Multi-Time Attention:} Using a single time attention network requires selecting a particular time embedding function $\phi(t)$ and projection matrices $W^Q$ and $W^K$. To make the model more expressive, we can use $H$ time embeddings and multiple sets of projection matrices to produce multiple interpolations, which can then be combined together. We let $\phi_h(t)$, $W_h^Q$ and $W_h^K$ be the time embedding and projection matrices for time embedding $h$. 
We let $\hat{x}_{hd}(t, \mbf{s})$ be the interpolant for dimension $d$ of time embedding $h$. 

The final output of the multi-time attention model is given by $\mbf{C}(t,\mbf{s})=[\mbf{C}_1(t,\mbf{s}),...,\mbf{C}_J(t,\mbf{s})]$ as defined below where $W_{hdj}^o$ is an $H\times D\times J$ projection tensor that defines a final $J$ dimensional latent space. This final latent space mixes information across all time embeddings $h$ and all data dimensions $d$ at each time point $t$.
%
\begin{align}
    C_{j}(t,\mbf{s}) = \sum_{h=1}^H\sum_{d=1}^D \hat{x}_{hd}(t, \mbf{s}) \cdot W_{hdj}^o 
\end{align}
%
Thus, the multi-time attention network takes an irregularly observed multi-variate time series as input and re-represents it in terms of a continuous multivariate function of time $\mbf{C}(t,\mbf{s})$ that mixes together information across time and input dimensions. To be useful for down-stream tasks, the function $\mbf{C}(t,\mbf{s})$ must be converted to a fixed-length representation. To do so, we first define a set of $T$ reference time points $\mbf{r} = [r_1, \cdots, r_T]$. We then evaluate $\mbf{C}(t,\mbf{s})$ at these points. This results in a length $T$ sequence of $J$ dimensional vectors $\mbf{c}=[\mbf{c}_1,...,\mbf{c}_T]$ with $\mbf{c}_i= \mbf{C}(t_i,\mbf{s})$. We refer to the function that maps an input time series $\mbf{s}$ to the fixed dimensional representation $\mbf{c}$ for a given set of reference points $\mbf{r}$ as $\mbf{c}=\text{mTAN}(\mbf{r},\mbf{s})$. This can be thought of as a highly specialized neural network module that can be further composed with standard recurrent or convolutional models as well and encoder-decoder-style generative models. 
In the next section, we describe the application of an encoder-decoder model.

%Multi Time Attention allows the model to learn multiple interpolations, each using different time embeddings. It is equivalent to learning interpolations with different kernels. Multi Time Attention is defined as:
%
%\begin{align}
%    \text{MTAF}(Q, K, V) &= \text{Concat} (I_1, \cdots, I_h) \,W^O \\
%    \text{where } I_k &= \text{TAF}_{W_k} (Q, K, V) \nonumber
%\end{align}
%
%where $W_k = \{W_k^Q \in \mathbb{R}^{d_k \times d}, W_k^K \in \mathbb{R}^{d_k \times d}\}$ and $W^O \in \mathbb{R}^{hD \times d_o}$ are parameter matrices defining the linear projections and $d, d_o$ are model hyperparameters.

%{\bf Special case:} For the case with single interpolation $h=1$, if the final projection is defined in the same space i.e., $W^O \in \mathbb{R}^{D \times D}$ then it is equivalent to merging information across all $D$ time series at each reference time point by taking into account learnable correlations across each dimension.

%looks similar to scaled dot product attention from cite paper but its not.

% Write theorem proving that the TAN actually learns a kernel function
% Because of the similarity of our model to scaled dot product attention, we call this Time Attention Network.

\paragraph{Encoder-Decoder Framework:}
\label{sec:enc-dec}
We define an encoder-decoder model based on 
combining the Multi-Time Attention module with recurrent networks. 
The encoder consists of three stages. An mTAN module is first used to map a raw sparse and irregularly sampled time series $\mbf{s}$ into a fixed-length mTAN representation $\mbf{c}^{enc}$ using a set of reference time points $\mbf{r}$ as described in the last section. Next, we apply an RNN encoder $\text{RNN}^{enc}$ that takes the sequence values $\mbf{c}_i^{enc}$ as inputs and produces latent states $\mbf{h}_i^{enc}$ as outputs (we define $\mbf{h}_0^{enc}=0$). In our experiments, we use a GRU-based encoder. Finally, we define a probability distribution at each reference time $r_i$ via $q(\mbf{z}_i| \mbf{h}_i^{enc})$. In our experiments,we chose the latent distribution $q(\mbf{z}_k| \mbf{h}_k^{enc})$ to be a diagonal Gaussian $\mathcal{N}(\bm{\mu}_i,
\bm{\sigma}_i^2)$ where $\bm{\mu}_i$ and $\bm{\sigma}_i^2$ are computed using a pair of fully
connected networks:
    $\bm{\mu}_i = f^{enc}_\mu(\mbf{h}_i^{enc})$ and 
     $\bm{\sigma}^2_i = \exp (f^{enc}_\sigma(\mbf{h}_i^{enc}))$.
We define $\mbf{z}=[\mbf{z}_1,...,\mbf{z}_T]$.
     
%Let $\text{ {MTAN}}^{enc}, \text{ {MTAN}}^{dec}$  be the encoder and decoder
%multi time attention network and
%$\text{RNN}^{enc}, \text{RNN}^{dec}$ be the function enacted by encoder
%and decoder recurrent network
%at a single time-step. The multi time attention network $\text{ {MTAN}}^{enc}$
%takes irregularly sampled time series as input and outputs a context vector 
%$\mbf{c}_k^{enc}$ at each query point $r_k$. %$\text{RNN}^{enc}$ takes the
%context vector $\mbf{c}_k^{enc}$ as input and outputs a hidden vector $\mbf{h}_k^{enc}$
%corresponding to the $k^{th}$ reference point $r_k$. The output of the
%encoder $\mbf{h}_k^{enc}$ is then used to parameterize a distribution $q(\mbf{z}_k|
%\mbf{h}_k^{enc})$ over the latent vector $\mbf{z}_k$. In our experiments, we chose
%latent distribution to be a diagonal Gaussian $\mathcal{N}(\bm{\mu}_k,
%\bm{\sigma}_k^2)$ where $\bm{\mu}_k$ and $\bm{\sigma}^2$ are computed using a fully
%connected network:
%
%\begin{align}
%    \bm{\mu}_k &= f^{enc}_\mu(\mbf{h}_k^{enc})\\
%     \bm{\sigma}^2_k &= \exp %(f^{enc}_\sigma(\mbf{h}_k^{enc}))
%\end{align}
%
At every reference point, the decoder takes a sample drawn from the latent distribution  $\mbf{z}_i \sim q(\mbf{z}_i| \mbf{h}_i^{enc})$  as input. An RNN decoder $\text{RNN}^{dec}$ takes the latent vector as input and outputs a hidden state  $\mbf{h}_i^{dec}$ (we define $\mbf{h}_0^{dec}=0$)
at each reference point $r_i$. We then apply an mTAN decoder to
produce mTAN latent states $\mbf{c}^{dec}_t$ at a collection of interpolation points. Finally, interpolations $\hat{\mbf{x}}^{dec}_t = f^{dec}(\mbf{c}_t^{dec})$ are then produced using a fully connected network $f^{dec}$.  

For a given irregularly sampled multivariate time series $\mbf{s} = (\mbf{t}, \mbf{x})$, the Encoder-Decoder framework performs the following computations to produce a mean interpolant $\hat{\mbf{x}}_t$:
%
\begin{align}
    \mbf{c}^{enc}_i &= \text{{mTAN}}^{enc} (r_i, \mbf{s})\\
    \mbf{h}^{enc}_i &= \text{RNN}^{enc}(\mbf{h}^{enc}_{i-1}, \mbf{c}^{enc}_i)\\
    \mbf{z}_i &\sim q(\mbf{z}_i| h_i^{enc})\\
    \mbf{h}_i^{dec} &= \text{RNN}^{dec} (\mbf{h}_{i-1}^{dec}, \mbf{z}_i)  \\
    \mbf{c}^{dec}_t &= \text{mTAN}^{dec} (t,(\mbf{r},\mbf{h}^{dec}))\\
    \hat{\mbf{x}}_t &= f^{dec}(\mbf{c}^{dec}_t)
    %\hat{\mbf{x}}_t &\sim p(\mbf{x}_t | f^{dec}(\mbf{c}^{dec}_t)) 
\end{align}
%
%$h^{enc}_0$ and $h^{dec}_0$ are initialized to zero.
%Note that the input to the encoder $\text{ {MTAN}}^{enc}$ is irregularly sampled data, we pack them into a fixed length sequence using mask variables as described in section \ref{sec:tan}. We donot need any mask for the decoder $\text{ {MTAN}}^{dec}$ as it takes fixed length vectors defined on fixed set of reference points as input. 

The corresponding generative process for a single data case sampled from our decoder network is shown below. Note that the generative process conditions on a set of query time points $\mbf{t} = \{t_1, \cdots, t_L\}$. We do not model the distribution over observation time points in this work.
%
\begin{align}
   \mbf{z}_k &\sim p(\mbf{z}_k)\\
    \mbf{h}_k^{dec} &= \text{RNN}^{dec} (\mbf{h}_{k-1}^{dec}, \mbf{z}_k)  \\
    \mbf{c}^{dec}_t &= \text{mTAN}^{dec} (t,(\mbf{r},\mbf{h}^{dec}))\\
    {\mbf{x}}_t &\sim p(\mbf{x}_t | f^{dec}(\mbf{c}^{dec}_t))
\end{align}
%
Here, each $z_k$ is sampled from the prior distribution $p(\mbf{z}_k)$ which is defined to be a standard multivariate normal distribution. 
The distribution $p(\mbf{x}_t | f^{dec}(\mbf{c}^{dec}_t))$ is also typically a simple distribution such as a diagonal covariance multivariate normal.

\paragraph{Learning}
%Derive the equations
To learn the parameters of our encoder and decoder model, we follow the standard VAE training approach to maximize a variational 
lower bound on the log marginal likelihood, also known as the evidence lower bound or ELBO. Let the encoder and decoder parameters be $\theta$ and $\gamma$ respectively, then the ELBO is defined as:
%
\begin{align}
 \mathcal{L}_{\text{VAE}} (\theta, \gamma) &= \sum_{n=1}^N\Big(\mathbb{E}_{q_{\gamma}(\mbf{z}|\mbf{s}_n)} [\log p_{\theta}(\mbf{x}_n| \mbf{z}, \mbf{t}_n) ] -  \KL(q_{\gamma}(\mbf{z} | \mbf{x}_n, \mbf{t}_n) || p(\mbf{z}))\Big) \\
\KL(q_{\gamma}(\mbf{z} | \mbf{x}_n, \mbf{t}_n) || p(\mbf{z})) & = \sum_{i=1}^T \KL(q_{\gamma}(\mbf{z}_i | \mbf{x}_n, \mbf{t}_n) || p(\mbf{z}_i))\\
\label{eq:lik}
\log p_{\theta}(\mbf{x}_n|\mbf{z}, \mbf{t}_n) &= \sum_{d=1}^{D}\sum_{j=1}^{L_{dn}} \log p_{\theta}(\mbf{x}_{jdn} | \mbf{z}, t_{jdn})
\end{align}
%
Since irregularly sampled time series can have different number of observations across different dimensions as well as across different data cases, it can be helpful to further normalize the terms in the objective function to avoid the model focusing on more accurately modeling sequences that are longer at the expense of sequences that are shorter. We propose a length-normalized objective to deal with this issue, as shown below. 
%One interpretation of this modification is that we are learning a family of models, one for each possible input sequence length $L_n$, while tying the parameters of these models together. 
%
\begin{align}
\mathcal{L}_{\text{NVAE}} (\theta, \gamma) = \sum_{n=1}^N \;\frac{1}{ \sum_d L_{dn}}\Big(\mathbb{E}_{q_{\gamma}(\mbf{z}|\mbf{s}_n} [\log p_{\theta}(\mbf{x}_n| \mbf{z},\mbf{t}_n) ] 
-  \KL(q_{\gamma}(\mbf{z} | \mbf{s}_n) || p(\mbf{z}))\Big) 
\end{align}
%
In practice, we use $k$ samples from the variational distribution $q_{\gamma}(\mbf{z}|\mbf{s}_n)$ to compute the learning objective.



% \subsection{Implementation Details}
